Vec2Sent: Probing Sentence Embeddings with Natural Language Generation

We introspect black-box sentence embeddings by conditionally generating from them with the objective to retrieve the underlying discrete sentence. We perceive of this as a new unsupervised probing task and show that it correlates well with downstream task performance. We also illustrate how the language generated from different encoders differs. We apply our approach to generate sentence analogies from sentence embeddings.

==> figures/tables/analogies.tex <==
\begin{table}[!htb]
    \centering
    \begin{tabular}{l|llll}
         \toprule
         \iffalse
         & \textbf{he visits italy}&  \textbf{he eats pizza} & & \textbf{she drinks wine}\\
         QT & & & she visits france &\\  
         LASER & & & she visits italy &\\
         SBERT & & & she travels spain &\\
         Avg & & & rate is & \\ \midrule
         & \textbf{he is a doctor}&  \textbf{his name is robert} & & \textbf{her name is julia}\\
         QT & & & she is a doctor &\\ 
         LASER &&& she is a nurse &\\
         SBERT && & she is medicine & \\
         Avg &&& a.i. &\\
         \fi 
         QT & she visits france & she is a doctor \\
         LASER & she visits italy & she is a nurse\\
         SBERT & she travels spain & she is medicine\\
         Avg & rate is & a.i.\\
         \bottomrule
    \end{tabular}
    \caption{Sentence level analogies $a:b\,\,::\,\, x:c$ for the triples ($a=$ he visits italy, $b=$ he eats pizza, $c=$  she drinks wine) on the left, and ($a=$ he is a doctor, $b=$ his name is robert, $c=$ her name is julia) on the right.}
    \label{table:analogies}
\end{table}

==> figures/tables/ranks.tex <==
\begin{table}[]
    \centering
    {\small
    \begin{tabular}{l|cc|cc} \toprule
         \textbf{Embedder} & \textbf{MR} & \textbf{TREC} & \textbf{Mover} & \textbf{Id}\\
         \midrule 
         Avg &  6 & 6 & 4 & 9\\
         GEM & 9 & 8 & 9 & 7\\
         Hier & 8 & 9 & 6 & 6\\
         Avg$+$Max$+$Hier & 7 & 7 & 5 & 8\\
         Sent2Vec & 4 & 5 & 7 & 5\\ \midrule
         InferSent & 3 & 2 & 2 & 3\\
         QuickThought & 2 & 1 & 3 & 4\\
         LASER & 5 & 3 & 1 & 1\\
         SBERT & 1 & 4 & 8 & 2\\
         \bottomrule
    \end{tabular}
    }
    \caption{Ranks}
    \label{tab:my_label}
\end{table}

==> figures/tables/top3.tex <==
\begin{table}[!htb]
    \input{top3_main}
    \caption{Encoders, their dimensionalities, and rank of encoders according to downstream (DS) and Vec2Sent diagnostic tasks. Ranks are calculated after averaging over all tasks.}
    \label{tab:top3}
\end{table}

==> related.tex <==
\section{Related work}
%Probing sentence embeddings has started with \citet{Adi.2017} or earlier, but \citet{Conneau.2018a} systematized terminology and datasets for sentence level probing tasks. 
The goal of probing tasks is to make the opaque embedding space $\mathbb{R}^d$ ``linguistically'' observable to humans. A plethora of different probing tasks have been suggested %by different authors
\citep{Adi.2017,Naik.2018,Linzen.2016,Shi.2016}, which \citet{Conneau.2018a} classify into \emph{surface}, \emph{syntactic}, and \emph{semantic} probing tasks. 
More recently, word level probing for especially contextualized representations  \citep{Tenney.2019,liu-etal-2019-linguistic} have been  investigated, along with first multilingual extensions of probing tasks \citep{Krasnowska.2019,Sahin.2019}. 

There are two ways to perceive of V2S: either as a new direct form of introspection of sentence embeddings. In this interpretation, V2S is somewhat similar to nearest neighbor overlap (N2O) as recently proposed in \citet{Lin:2019}. N20 compares two encoders by their overlap in nearest neighbor sentences for a given query sentence. Our model does not search for nearest neighbors in a sentence space, but directly generates the ``nearest neighbor'' for a given input sentence (embedding). Alternatively, V2S may be seen as a novel, additional probing task that complements the traditional canon of probing tasks. In this view, V2S is most closely related to the word content (WC) probing task, which asks %to check 
whether an embedding stores a certain query word. V2S is much more challenging: it asks to retrieve all the words of a sentence and put them into the correct word order. 
%As such, we would expect that vec2sent has considerably higher discriminative power compared to WC.  
%Comparability: nearest neighbors

==> trec.tex <==
\section{TrecQA}
\begin{table}
\begin{tabular}{c c c c}
  & Who & Where & When\\
  LASER & 64.92 & 70.56 & 65.99\\
  Infersent & 63.33 & 72.18 & 67.70\\
  Quickthought & 63.51 & 75.82 & 66.54\\
  SBERT & 64.04 & 67.19 & 63.35\\
  \hline
  Average & 61.86 & 63.14 & 62.37\\
  Hier & 65.85 & 68.70 & 63.91\\
  Avg+Max+Hier & 65.49 & 63.87 & 64.20\\
\end{tabular}
\caption{Average Mover Scores}
\end{table}
